A Universal Systematic Method to Generate Error Patterns on Memoryless Channels

The high computational cost of approaching the performance of Maximum-likelihood (ML) decoding has limited its practical use for decades. Because the complexity grows exponentially with the message length, researchers have spent years developing algorithms like Ordered Statistics Decoding (OSD), Partial Ordered Statistics Decoding (POSD) and Guessing Random Additive Noise decoding (GRAND) which try to approach ML performance. OSD, POSD and GRAND work by trying to guess the error patterns affecting the received signals. However, there does not exist a systematic method to extend the error pattern guesses to novel channels. This work introduces a systematic method that uses the Probability Density Function (PDF) of a memoryless channel to generate a set of error patterns that can be applied on any future received signal on this channel. Simulation results show that our proposed method applied on GRAND, OSD and POSD generally matches or outperforms current pre-generated error patterns on additive white Gaussian noise (AWGN) channel, mixture of Gaussian distribution channels, Rayleigh fading channel with perfect knowledge of Channel State Information (CSI) and Rayleigh fading channel with no perfect knowledge of Channel State Information (NCSI).

==> Figures/AWGN/Simulations/performance_grand.tex <==
% \begin{figure}[!t]
%   \centering
%   \begin{tikzpicture}[]
%     \begin{groupplot}[group style={group name=fer_queries, group size= 2 by 1, horizontal sep=5pt, vertical sep=5pt},
%       footnotesize,
%       height=.6\columnwidth,  width=0.80\columnwidth,  
%       xlabel=$\frac{E_b}{N_0}$,
%       ymode=log,
%       tick align=inside,
%       grid=both, grid style={gray!30},
%       /pgfplots/table/ignore chars={|},
%       ] % mark options={scale=1.5}
%       \nextgroupplot[ylabel= FER, ytick pos=left, y label style={at={(axis description cs:-0.225,.5)},anchor=south},ymin=1e-6, ymax = 1, xmin=1, xmax=10]
%     \addplot[mark=square, Paired-3 , semithick]  table[x=Eb/N0, y=FER] {Figures/AWGN/Simulations/RLC_127_85_GRAND_EW_0_1_10_MQ_1000000_SIM_mHW_127_AWGN.res}; \label{gp:AWGN_GRAND_EW_perf}
%        \addplot[mark=triangle  , Paired-6, semithick]  table[x=Eb/N0, y=FER] {Figures/AWGN/Simulations/RLC_127_85_GRAND_HW_0_1_10_MQ_1000000_SIM_mHW_127_AWGN.res} ;\label{gp:AWGN_GRAND_HW_perf}
%          \addplot[mark=otimes  , Paired-9, semithick]  table[x=Eb/N0, y=FER] {Figures/AWGN/Simulations/RLC_127_85_GRAND_LW_0_1_10_MQ_1000000_SIM_mHW_127_AWGN.res} ;\label{gp:AWGN_GRAND_LW_perf}
%      \addplot[mark=-, cyan , semithick]  table[x=Eb/N0, y=FER] {Figures/AWGN/Simulations/RLC_127_85_GRAND_ILW_0_1_10_MQ_1000000_SIM_mHW_127_AWGN.res};\label{gp:AWGN_GRAND_ILW_perf}
%        \addplot[mark=+  , teal, dashed]  table[x=Eb/N0, y=FER] {Figures/AWGN/Simulations/BCH_127_85_GRAND_ISTEP_0_1_10_MQ_1000_SIM_mHW_127_AWGN.res} ;\label{gp:AWGN_GRAND_ISTEP_perf}
%         \addplot[mark=square, Paired-3 , dashed]  table[x=Eb/N0, y=FER] {Figures/AWGN/Simulations/BCH_127_85_GRAND_EW_0_1_10_MQ_1000_SIM_mHW_127_AWGN.res}; 
%        \addplot[mark=triangle  , Paired-6, dashed]  table[x=Eb/N0, y=FER] {Figures/AWGN/Simulations/BCH_127_85_GRAND_HW_0_1_10_MQ_1000_SIM_mHW_127_AWGN.res} ;
%          \addplot[mark=otimes  , Paired-9, dashed]  table[x=Eb/N0, y=FER] {Figures/AWGN/Simulations/BCH_127_85_GRAND_LW_0_1_10_MQ_1000_SIM_mHW_127_AWGN.res} ;
%          \addplot[mark=o, cyan , dashed]  table[x=Eb/N0, y=FER] {Figures/AWGN/Simulations/RLC_127_85_GRAND_ILW_0_1_10_MQ_1000_SIM_mHW_127_AWGN.res};
%       \coordinate (top) at (rel axis cs:0,1);
%       \coordinate (spypoint1) at (axis cs:7.45,2e-7);
%       \coordinate (magnifyglass1) at (axis cs:2.6,1.1e-5);
%       \coordinate (bot) at (rel axis cs:1,0);
%     \end{groupplot}
%     \path (top|-current bounding box.north) -- coordinate(legendpos) (bot|-current bounding box.north);
%     \matrix[
%     matrix of nodes,
%     anchor=south,
%     draw,
%     inner sep=0.2em,
%     draw
%     ]at(legendpos) %% heer
%     {
%     \ref{gp:AWGN_GRAND_EW_perf}& \tiny  EW &[1pt] 
%     \ref{gp:AWGN_GRAND_LW_perf}& \tiny  LW &[1pt] \ref{gp:AWGN_GRAND_HW_perf}& \tiny  HW &[1pt] \ref{gp:AWGN_GRAND_ILW_perf}& \tiny  ILW &[1pt]  \ref{gp:AWGN_GRAND_ISTEP_perf}& \tiny  ISTEP &[1pt] \\
%       };
%       % \spy [blue, width=1.25cm, height=1.25cm] on (spypoint1) in node[fill=white] at (magnifyglass1); 
%   \end{tikzpicture}
%   \vspace*{-1em}
%   \caption{ Comparison of decoding performance of different error patterns with GRAND on RLC (127,85). Straight lines correspond to simulations with maximum number of queries of $10^6$ while dashed lines correspond to simulations with maximum number of queries of $10^3$}\label{fig:performance_grand_awgn}
%    \vspace*{-1.3em}
% \end{figure}

==> Figures/AWGN/Simulations_OSD/performance_osd.tex <==
% \begin{figure}[!t]
%   \centering
%   \begin{tikzpicture}[]
%     \begin{groupplot}[group style={group name=fer_queries, group size= 2 by 1, horizontal sep=5pt, vertical sep=5pt},
%       footnotesize,
%       height=.6\columnwidth,  width=0.80\columnwidth,  
%       xlabel=$\frac{E_b}{N_0}$,
%       ymode=log,
%       tick align=inside,
%       grid=both, grid style={gray!30},
%       /pgfplots/table/ignore chars={|},
%       ] % mark options={scale=1.5}
%       \nextgroupplot[ylabel= FER, ytick pos=left, y label style={at={(axis description cs:-0.225,.5)},anchor=south},ymin=1e-6, ymax = 1, xmin=1, xmax=10]
%     \addplot[mark=square, Paired-3 , semithick]  table[x=Eb/N0, y=FER] {Figures/AWGN/Simulations_OSD/BCH_127_64_OSD_EW_0_1_10_MQ_1000_SIM_mHW_127_AWGN.res}; \label{gp:AWGN_OSD_EW_perf}
%        \addplot[mark=triangle, Paired-6, semithick]  table[x=Eb/N0, y=FER] {Figures/AWGN/Simulations_OSD/BCH_127_64_OSD_HW_0_1_10_MQ_1000_SIM_mHW_127_AWGN.res} ;\label{gp:AWGN_OSD_HW_perf}
%          \addplot[mark=otimes, Paired-9, semithick]  table[x=Eb/N0, y=FER] {Figures/AWGN/Simulations_OSD/BCH_127_64_OSD_LW_0_1_10_MQ_1000_SIM_mHW_127_AWGN.res} ;\label{gp:AWGN_OSD_LW_perf}
%      \addplot[mark=-, cyan , semithick]  table[x=Eb/N0, y=FER] {Figures/AWGN/Simulations_OSD/BCH_127_64_OSD_ILW_0_1_10_MQ_1000_SIM_mHW_127_AWGN.res};\label{gp:AWGN_OSD_ILW_perf}
%        % \addplot[mark=+  , teal, dashed]  table[x=Eb/N0, y=FER] {Figures/AWGN/Simulations_OSD/BCH_127_64_OSD_ISTEP_0_1_10_MQ_1000_SIM_mHW_127_AWGN.res} ;\label{gp:AWGN_OSD_ISTEP_perf}
%        %  \addplot[mark=square, Paired-3 , dashed]  table[x=Eb/N0, y=FER] {Figures/AWGN/Simulations_OSD/BCH_127_64_OSD_EW_0_1_10_MQ_1000_SIM_mHW_127_AWGN.res}; 
%        % \addplot[mark=triangle  , Paired-6, dashed]  table[x=Eb/N0, y=FER] {Figures/AWGN/Simulations_OSD/BCH_127_64_OSD_HW_0_1_10_MQ_1000_SIM_mHW_127_AWGN.res} ;
%        %   \addplot[mark=otimes  , Paired-9, dashed]  table[x=Eb/N0, y=FER] {Figures/AWGN/Simulations_OSD/BCH_127_64_OSD_LW_0_1_10_MQ_1000_SIM_mHW_127_AWGN.res} ;
%        %   \addplot[mark=-, cyan , dashed]  table[x=Eb/N0, y=FER] {Figures/AWGN/Simulations_OSD/BCH_127_64_OSD_ILWO_0_1_10_MQ_1000_SIM_mHW_127_AWGN.res};
%       \coordinate (top) at (rel axis cs:0,1);
%       \coordinate (spypoint1) at (axis cs:7.45,2e-7);
%       \coordinate (magnifyglass1) at (axis cs:2.6,1.1e-5);
%       \coordinate (bot) at (rel axis cs:1,0);
%     \end{groupplot}
%     \path (top|-current bounding box.north) -- coordinate(legendpos) (bot|-current bounding box.north);
%     \matrix[
%     matrix of nodes,
%     anchor=south,
%     draw,
%     inner sep=0.2em,
%     draw
%     ]at(legendpos) %% heer
%     {
%     \ref{gp:AWGN_OSD_EW_perf}& \tiny  EW &[1pt] 
%     \ref{gp:AWGN_OSD_LW_perf}& \tiny  LW &[1pt] \ref{gp:AWGN_OSD_HW_perf}& \tiny  HW &[1pt] \ref{gp:AWGN_OSD_ILW_perf}& \tiny  ILW &[1pt]  \ref{gp:AWGN_OSD_ISTEP_perf}& \tiny  ISTEP &[1pt] \\
%       };
%       % \spy [blue, width=1.25cm, height=1.25cm] on (spypoint1) in node[fill=white] at (magnifyglass1); 
%   \end{tikzpicture}
%   \vspace*{-1em}
%   \caption{ Comparison of decoding performance of different error patterns with OSD on BCH (127,64). Straight lines correspond to simulations with maximum number of queries of $10^4$.}
%    \vspace*{-1.3em}
% \end{figure}

==> Figures/AWGN/expected_values_128_osd_latex.tex <==
% x y
64 6.29168512552301
65 6.36108093320757
66 6.4304997951733
67 6.49996761318505
68 6.56951045906342
69 6.63915464116153
70 6.70892677270615
71 6.7788538424751
72 6.84896328827836
73 6.91928307379447
74 6.98984176932254
75 7.0606686370846
76 7.13179372177677
77 7.20324794713727
78 7.27506321939288
79 7.34727253855259
80 7.41991011863206
81 7.49301151804485
82 7.56661378155765
83 7.64075559541112
84 7.71547745743662
85 7.79082186427953
86 7.86683351816503
87 7.94355955603609
88 8.02104980434824
89 8.09935706337685
90 8.1785374255514
91 8.2586506331444
92 8.33976048162041
93 8.42193527615119
94 8.50524835026106
95 8.58977865737239
96 8.67561144825008
97 8.76283905013233
98 8.85156176680257
99 8.94188892327609
100 9.03394008434365
101 9.12784648338639
102 9.22375270709742
103 9.32181869378649
104 9.42222211874707
105 9.52516126111825
106 9.63085847485148
107 9.73956442451255
108 9.8515632991344
109 9.96717929033031
110 10.0867847240419
111 10.2108103834883
112 10.3397587773231
113 10.4742214297115
114 10.6149017602726
115 10.7626458882604
116 10.918484923682
117 11.0836943383032
118 11.2598794848297
119 11.4491025275215
120 11.6540776252267
121 11.8784840926167
122 12.1274956637789
123 12.4087352340304
124 12.7341487082727
125 13.1241265889609
126 13.6181827444618
127 14.310854717746
128 15.5523937235798


==> Figures/AWGN/timing/mine.tex <==
EbNo    Timestamps
3   2.8560471
3.5 2.8814288
4   2.8944723
4.5 2.9345869
5   3.0093749
5.5 3.0340508
6   3.0966617
6.5 3.167356
7   3.2586001
7.5 3.3275692
8   3.5533029
8.5 3.6653762
9   3.771484


==> Figures/AWGN/timing/mine10k.tex <==
EbNo Timestamps
3   3.1212048
3.5 3.1467645
4   3.1635672
4.5 3.2026122
5   3.2779909
5.5 3.3054379
6   3.364733
6.5 3.438506
7   3.5303244
7.5 3.5945127
8   3.8219088
8.5 3.9393487
9   4.0461177


==> Figures/AWGN/timing/monte.tex <==
EbNo Timestamps
3   1240.0715161
3.5 367.8831
4   134.9793101
4.5 61.090468
5   36.0700357
5.5 28.9163817
6   29.7197297
6.5 44.3312612
7   93.2111496
7.5 284.493864
8   1277.2779814
8.5 8766.2415737
9   108564.23

==> Figures/AWGN/timing/monte10k.tex <==
EbNo Timestamps
3 4526.8975168
3.5   1607.9945095
4 706.4853199
4.5   409.7086601
5 317.616023
5.5   333.2398843
6 505.1291417
6.5   1114.7146785
7 3726.508313
7.5   19914.219513
8   173702.1209393


==> Figures/AWGN/whd_awgn_dist_hw_whd.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Figures/AWGN/HWWHD.eps}
    \caption{The weighted hamming distance as a function of error pattern index in the hamming weight generation sequence and in the optimal generation sequence.}
    \label{fig:whd_awgn_dist_hw_whd}
\end{figure}


==> Figures/AWGN/whd_awgn_dist_istep_ilwo.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Figures/AWGN/short.eps}
    \caption{The weighted hamming distance as a function of error pattern index in the improved step GRAND, improved logistic weight and optimal generation sequence.}
    \label{fig:whd_awgn_dist_istep_ilwo}
\end{figure}


==> Figures/AWGN/whd_awgn_dist_orb_whd.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Figures/AWGN/LWWHD.eps}
    \caption{The weighted hamming distance as a function of error pattern index in the hamming weight generation sequence and in the optimal generation sequence.}
    \label{fig:whd_awgn_dist_orb_whd}
\end{figure}

==> Figures/Comp_additive_fading/fading_comp.tex <==
numPatterns grand-f grand-fncsi posd-f posd-fncsi  osd-f  osd-fncsi
100 76 94 81 92 76 97
1000 63 90 73 92 61 99
10000 55 86 68 94 69 98
100000 47 83 65 95 71 96
1000000 42 81 64 96 66 94


==> Figures/Mixture_of_Gaussians/GRAND/EW.tex <==
% #-----------------------------------------------------------------
% # Decoder simulator (v3.0.2)
% #-----------------------------------------------------------------
% #
% ###### #### Simulate ###### ####
% #    ** Quantization  word length | decimal length       = -1 | -1
% #
% # * EW Error Patterns parameters: 
% #    ** Bit Locs       = 127
% #    ** Decoder        = GRAND
% #    ** Maximum Q      = 100
% #
% # * Initialize GRAND Decoding with the following code: 
% #    ** G_matrix_name       = ./Generators/BCH/BCH_G_127_106.txt
% #
% -------------- |-------|-------------- |-----------------|----------|----------|-----------------|----------|----------|----------|----------|----------|----------|
     MaxQ        | Eb/N0 |      Es/N0    |      FRA        |       BE |       FE |      QUE        |      BER |      FER |   QUE/FR | OQUE/FR  |  BOPs/FR | FLOPS/FR |
% -------------- |-------|---------------|-----------------|----------|----------|-----------------|----------|----------|----------|----------|----------|----------|
           100 |     5.00 |           4.22 |            398 |      244 |      100 |          13092 | 4.83e-03 | 2.51e-01 | 3.29e+01 | 3.29e+01 | 1.79e+05 | 8.87e+02 | 
          1000 |     5.00 |           4.22 |           1016 |      326 |      100 |         179314 | 2.53e-03 | 9.84e-02 | 1.76e+02 | 1.76e+02 | 9.60e+05 | 8.87e+02 | 
         10000 |     5.00 |           4.22 |           2894 |      339 |      100 |        1858342 | 9.22e-04 | 3.46e-02 | 6.42e+02 | 6.42e+02 | 3.49e+06 | 8.87e+02 | 
        100000 |     5.00 |           4.22 |          12141 |      443 |      100 |       23432877 | 2.87e-04 | 8.24e-03 | 1.93e+03 | 1.93e+03 | 1.05e+07 | 8.87e+02 | 
       1000000 |     5.00 |           4.22 |          46945 |      676 |      100 |      182191454 | 1.13e-04 | 2.13e-03 | 3.88e+03 | 3.88e+03 | 2.11e+07 | 8.87e+02 | 


==> Figures/Mixture_of_Gaussians/GRAND/RLC_127_85_GRAND_ML_0_5_5_MQ_1000_SIM_mHW_85_CUSTOM_2.tex <==
#-----------------------------------------------------------------
# Decoder simulator (v3.0.2)
#-----------------------------------------------------------------
#
###### #### Simulate ###### ####
#    ** Quantization  word length | decimal length       = -1 | -1
#
# * ML Error Patterns parameters: 
#    ** Decoder        = GRAND
#    ** Maximum HW     = 85
#    ** Maximum Q      = 1000
#
# * Initialize GRAND Decoding with the following code: 
#    ** G_matrix_name       = ./Generators/RLC/RLC_G_127_85.txt
#
% -------------- |-------|-------------- |-----------------|----------|----------|-----------------|----------|----------|----------|----------|----------|----------|
     MaxQ        | Eb/N0 |      Es/N0    |      FRA        |       BE |       FE |      QUE        |      BER |      FER |   QUE/FR | OQUE/FR  |  BOPs/FR | FLOPS/FR |
% -------------- |-------|---------------|-----------------|----------|----------|-----------------|----------|----------|----------|----------|----------|----------|
           100 |     5.00 |           3.26 |            352 |      258 |      100 |          12660 | 5.77e-03 | 2.84e-01 | 3.60e+01 | 3.60e+01 | 3.87e+05 | 6.27e+02 | 
          1000 |     5.00 |           3.26 |           1096 |      313 |      100 |         161826 | 2.25e-03 | 9.12e-02 | 1.48e+02 | 1.48e+02 | 1.59e+06 | 6.18e+02 | 
         10000 |     5.00 |           3.26 |           3805 |      330 |      100 |        1966607 | 6.83e-04 | 2.63e-02 | 5.17e+02 | 5.17e+02 | 5.56e+06 | 6.39e+02 | 
        100000 |     5.00 |           3.26 |          15347 |      410 |      100 |       22944148 | 2.10e-04 | 6.52e-03 | 1.50e+03 | 1.50e+03 | 1.61e+07 | 6.25e+02 | 
       1000000 |     5.00 |           3.26 |          77055 |      479 |      100 |      289633742 | 4.89e-05 | 1.30e-03 | 3.76e+03 | 3.76e+03 | 4.04e+07 | 6.26e+02 | 
# End of the simulation


==> Figures/Mixture_of_Gaussians/HOSD/EW_1C2.tex <==
% #-----------------------------------------------------------------
% # Decoder simulator (v3.0.2)
% #-----------------------------------------------------------------
% #
% ###### #### Simulate ###### ####
% #    ** Quantization  word length | decimal length       = -1 | -1
% #
% # * EW Error Patterns parameters: 
% #    ** Bit Locs       = 64
% #    ** Decoder        = HOSD
% #    ** Maximum Q      = 100
% #
% # * Initialize Simplified Ordered Statistics Decoding with the following code: 
% #    ** G_matrix_name       = ./Generators/BCH/G_127_64_10.txt
% #
% -------------- |-------|-------------- |-----------------|----------|----------|-----------------|----------|----------|----------|----------|----------|----------|
     MaxQ        | Eb/N0 |      Es/N0    |      FRA        |       BE |       FE |      QUE        |      BER |      FER |   QUE/FR | OQUE/FR  |  BOPs/FR | FLOPS/FR |
% -------------- |-------|---------------|-----------------|----------|----------|-----------------|----------|----------|----------|----------|----------|----------|
         %   100 |     5.00 |           2.02 |           1341 |     2661 |      100 |         105291 | 1.56e-02 | 7.46e-02 | 7.85e+01 | 2.34e+01 | 8.50e+06 | 1.77e+03 | 
         %  1000 |     5.00 |           2.02 |          13622 |     2549 |      100 |       10551074 | 1.47e-03 | 7.34e-03 | 7.75e+02 | 6.96e+01 | 3.44e+07 | 1.77e+03 | 
         % 10000 |     5.00 |           2.02 |          92362 |     2455 |      100 |      715400824 | 2.09e-04 | 1.08e-03 | 7.75e+03 | 1.65e+02 | 2.07e+08 | 1.77e+03 | 
                    100 |     5.00 |           2.02 |           1388 |     2635 |      100 |         107615 | 1.49e-02 | 7.20e-02 | 7.75e+01 | 2.26e+01 | 8.21e+06 | 1.77e+03 | 
          1000 |     5.00 |           2.02 |          11602 |     2543 |      100 |        8911693 | 1.73e-03 | 8.62e-03 | 7.68e+02 | 6.66e+01 | 3.33e+07 | 1.77e+03 | 
         10000 |     5.00 |           2.02 |         111700 |     2471 |      100 |      864715231 | 1.74e-04 | 8.95e-04 | 7.74e+03 | 1.56e+02 | 2.04e+08 | 1.77e+03 | 
        100000 |     5.00 |           2.02 |        1514891 |     2447 |      100 |   117235642538 | 1.27e-05 | 6.60e-05 | 7.74e+04 | 2.69e+02 | 1.98e+09 | 1.77e+03 | 
# End of the simulation

==> Figures/Mixture_of_Gaussians/HOSD/HW_1C2.tex <==
% #-----------------------------------------------------------------
% # Decoder simulator (v3.0.2)
% #-----------------------------------------------------------------
% #
% ###### #### Simulate ###### ####
% #    ** Quantization  word length | decimal length       = -1 | -1
% #
% # * HW Error Patterns Parameters: 
% #    ** Bit Locs       = 127
% #    ** Decoder        = HOSD
% #    ** List Size      = 10000000
% #    ** Minimum Q      = 1
% #    ** Step Q      = 1
% #    ** Maximum HW     = 127
% #    ** List Size      = 10000000
% #    ** Maximum Q      = 100
% #
% # * Initialize Simplified Ordered Statistics Decoding with the following code: 
% #    ** G_matrix_name       = ./Generators/BCH/G_127_64_10.txt
% #
% -------------- |-------|-------------- |-----------------|----------|----------|-----------------|----------|----------|----------|----------|----------|----------|
     MaxQ        | Eb/N0 |      Es/N0    |      FRA        |       BE |       FE |      QUE        |      BER |      FER |   QUE/FR | OQUE/FR  |  BOPs/FR | FLOPS/FR |
% -------------- |-------|---------------|-----------------|----------|----------|-----------------|----------|----------|----------|----------|----------|----------|
           100 |     5.00 |           2.02 |            137 |     2801 |      100 |          13737 | 1.61e-01 | 7.30e-01 | 1.00e+02 | 8.46e+01 | 2.80e+07 | 0.00e+00 | 
          1000 |     5.00 |           2.02 |            162 |     2659 |      100 |         160162 | 1.29e-01 | 6.17e-01 | 9.89e+02 | 7.39e+02 | 2.48e+08 | 0.00e+00 | 
         10000 |     5.00 |           2.02 |            237 |     2558 |      100 |        2370237 | 8.50e-02 | 4.22e-01 | 1.00e+04 | 4.97e+03 | 1.75e+09 | 0.00e+00 | 
        100000 |     5.00 |           2.02 |            446 |     2564 |      100 |       44300446 | 4.53e-02 | 2.24e-01 | 9.93e+04 | 3.18e+04 | 1.20e+10 | 0.00e+00 | 
# End of the simulation


==> Figures/Mixture_of_Gaussians/HOSD/ILW_1C2.tex <==
% #-----------------------------------------------------------------
% # Decoder simulator (v3.0.2)
% #-----------------------------------------------------------------
% #
% ###### #### Simulate ###### ####
% #    ** Quantization  word length | decimal length       = -1 | -1
% #
% # * ILW Error Patterns Parameters: 
% #    ** Bit Locs       = 127
% #    ** List Size      = 10000000
% #    ** Minimum Q      = 1
% #    ** Step Q      = 1
% #    ** Decoder        = ILW
% #    ** Maximum Q      = 100
% #
% # * Initialize Simplified Ordered Statistics Decoding with the following code: 
% #    ** G_matrix_name       = ./Generators/BCH/G_127_64_10.txt
% #
% -------------- |-------|-------------- |-----------------|----------|----------|-----------------|----------|----------|----------|----------|----------|----------|
     MaxQ        | Eb/N0 |      Es/N0    |      FRA        |       BE |       FE |      QUE        |      BER |      FER |   QUE/FR | OQUE/FR  |  BOPs/FR | FLOPS/FR |
% -------------- |-------|---------------|-----------------|----------|----------|-----------------|----------|----------|----------|----------|----------|----------|
           100 |     5.00 |           2.02 |            177 |     2772 |      100 |          17601 | 1.23e-01 | 5.65e-01 | 9.94e+01 | 9.14e+01 | 3.04e+07 | 8.87e+02 | 
          1000 |     5.00 |           2.02 |            302 |     2662 |      100 |         300002 | 6.94e-02 | 3.31e-01 | 9.93e+02 | 7.11e+02 | 2.43e+08 | 8.87e+02 | 
         10000 |     5.00 |           2.02 |            670 |     2616 |      100 |        6660004 | 3.07e-02 | 1.49e-01 | 9.94e+03 | 4.83e+03 | 1.73e+09 | 8.87e+02 | 
        100000 |     5.00 |           2.02 |           2240 |     2636 |      100 |      222500015 | 9.27e-03 | 4.46e-02 | 9.93e+04 | 2.57e+04 | 1.04e+10 | 8.87e+02 | 
# End of the simulation


==> Figures/Mixture_of_Gaussians/HOSD/LW_1C2.tex <==
% #-----------------------------------------------------------------
% # Decoder simulator (v3.0.2)
% #-----------------------------------------------------------------
% #
% ###### #### Simulate ###### ####
% #    ** Quantization  word length | decimal length       = -1 | -1
% #
% # * LW Error Patterns Parameters: 
% #    ** Bit Locs       = 64
% #    ** Decoder        = HOSD
% #    ** List Size      = 10000000
% #    ** Maximum Q      = 100
% #    ** Minimum Q      = 1
% #    ** Step Q      = 100
% #    ** Maximum HW     = 127
% #    ** LW max         = 128
% #
% # * Initialize Simplified Ordered Statistics Decoding with the following code: 
% #    ** G_matrix_name       = ./Generators/BCH/G_127_64_10.txt
% #
% -------------- |-------|-------------- |-----------------|----------|----------|-----------------|----------|----------|----------|----------|----------|----------|
     MaxQ        | Eb/N0 |      Es/N0    |      FRA        |       BE |       FE |      QUE        |      BER |      FER |   QUE/FR | OQUE/FR  |  BOPs/FR | FLOPS/FR |
% -------------- |-------|---------------|-----------------|----------|----------|-----------------|----------|----------|----------|----------|----------|----------| 
           100 |     5.00 |           2.02 |           1315 |     2677 |      100 |         102691 | 1.60e-02 | 7.60e-02 | 7.81e+01 | 2.14e+01 | 7.84e+06 | 3.84e+02 | 
          1000 |     5.00 |           2.02 |           3208 |     2537 |      100 |        2490718 | 6.23e-03 | 3.12e-02 | 7.76e+02 | 8.97e+01 | 4.22e+07 | 3.84e+02 | 
         10000 |     5.00 |           2.02 |          35169 |     2517 |      100 |      272337936 | 5.64e-04 | 2.84e-03 | 7.74e+03 | 2.07e+02 | 2.40e+08 | 3.84e+02 | 
        100000 |     5.00 |           2.02 |         342175 |     2409 |      100 |    26473877437 | 5.54e-05 | 2.92e-04 | 7.74e+04 | 3.51e+02 | 2.23e+09 | 3.84e+02 | 
       % 1000000 |     5.00 |           2.02 |        5988106 |     2408 |      100 |  4631948356159 | 3.17e-06 | 1.67e-05 | 7.74e+05 | 4.83e+02 | 2.53e+10 | 3.84e+02 | 

==> Figures/Mixture_of_Gaussians/HOSD/pdf_hosd_n.tex <==
x pdf
-5.000000 0.000406
-4.989990 0.000450
-4.979980 0.000498
-4.969970 0.000551
-4.959960 0.000609
-4.949950 0.000673
-4.939940 0.000743
-4.929930 0.000819
-4.919920 0.000902
-4.909910 0.000994
-4.899900 0.001093
-4.889890 0.001202
-4.879880 0.001320
-4.869870 0.001449
-4.859860 0.001589
-4.849850 0.001741
-4.839840 0.001906
-4.829830 0.002085
-4.819820 0.002280
-4.809810 0.002490
-4.799800 0.002718
-4.789790 0.002964
-4.779780 0.003230
-4.769770 0.003517
-4.759760 0.003826
-4.749750 0.004160
-4.739740 0.004518
-4.729730 0.004904
-4.719720 0.005319
-4.709710 0.005764
-4.699700 0.006242
-4.689690 0.006753
-4.679680 0.007301
-4.669670 0.007887
-4.659660 0.008513
-4.649650 0.009182
-4.639640 0.009895
-4.629630 0.010656
-4.619620 0.011465
-4.609610 0.012327
-4.599600 0.013242
-4.589590 0.014215
-4.579580 0.015246
-4.569570 0.016340
-4.559560 0.017498
-4.549550 0.018723
-4.539540 0.020018
-4.529530 0.021386
-4.519520 0.022830
-4.509510 0.024351
-4.499499 0.025953
-4.489489 0.027639
-4.479479 0.029411
-4.469469 0.031271
-4.459459 0.033223
-4.449449 0.035269
-4.439439 0.037411
-4.429429 0.039652
-4.419419 0.041994
-4.409409 0.044439
-4.399399 0.046989
-4.389389 0.049645
-4.379379 0.052411
-4.369369 0.055286
-4.359359 0.058273
-4.349349 0.061373
-4.339339 0.064587
-4.329329 0.067915
-4.319319 0.071358
-4.309309 0.074915
-4.299299 0.078588
-4.289289 0.082376
-4.279279 0.086278
-4.269269 0.090293
-4.259259 0.094420
-4.249249 0.098657
-4.239239 0.103003
-4.229229 0.107455
-4.219219 0.112011
-4.209209 0.116667
-4.199199 0.121420
-4.189189 0.126267
-4.179179 0.131204
-4.169169 0.136225
-4.159159 0.141327
-4.149149 0.146503
-4.139139 0.151748
-4.129129 0.157057
-4.119119 0.162423
-4.109109 0.167839
-4.099099 0.173298
-4.089089 0.178792
-4.079079 0.184315
-4.069069 0.189858
-4.059059 0.195412
-4.049049 0.200970
-4.039039 0.206521
-4.029029 0.212058
-4.019019 0.217571
-4.009009 0.223050
-3.998999 0.228486
-3.988989 0.233869
-3.978979 0.239189
-3.968969 0.244437
-3.958959 0.249601
-3.948949 0.254672
-3.938939 0.259641
-3.928929 0.264497
-3.918919 0.269229
-3.908909 0.273830
-3.898899 0.278288
-3.888889 0.282595
-3.878879 0.286741
-3.868869 0.290717
-3.858859 0.294515
-3.848849 0.298126
-3.838839 0.301542
-3.828829 0.304756
-3.818819 0.307759
-3.808809 0.310546
-3.798799 0.313110
-3.788789 0.315445
-3.778779 0.317545
-3.768769 0.319406
-3.758759 0.321023
-3.748749 0.322393
-3.738739 0.323512
-3.728729 0.324377
-3.718719 0.324987
-3.708709 0.325341
-3.698699 0.325436
-3.688689 0.325273
-3.678679 0.324853
-3.668669 0.324177
-3.658659 0.323245
-3.648649 0.322061
-3.638639 0.320626
-3.628629 0.318945
-3.618619 0.317022
-3.608609 0.314860
-3.598599 0.312465
-3.588589 0.309843
-3.578579 0.306999
-3.568569 0.303940
-3.558559 0.300673
-3.548549 0.297206
-3.538539 0.293545
-3.528529 0.289700
-3.518519 0.285679
-3.508509 0.281490
-3.498498 0.277143
-3.488488 0.272647
-3.478478 0.268011
-3.468468 0.263245
-3.458458 0.258359
-3.448448 0.253363
-3.438438 0.248267
-3.428428 0.243080
-3.418418 0.237813
-3.408408 0.232475
-3.398398 0.227078
-3.388388 0.221630
-3.378378 0.216141
-3.368368 0.210621
-3.358358 0.205079
-3.348348 0.199525
-3.338338 0.193967
-3.328328 0.188415
-3.318318 0.182877
-3.308308 0.177361
-3.298298 0.171875
-3.288288 0.166426
-3.278278 0.161023
-3.268268 0.155671
-3.258258 0.150378
-3.248248 0.145150
-3.238238 0.139993
-3.228228 0.134912
-3.218218 0.129912
-3.208208 0.124998
-3.198198 0.120175
-3.188188 0.115447
-3.178178 0.110817
-3.168168 0.106288
-3.158158 0.101863
-3.148148 0.097545
-3.138138 0.093336
-3.128128 0.089238
-3.118118 0.085253
-3.108108 0.081380
-3.098098 0.077622
-3.088088 0.073979
-3.078078 0.070451
-3.068068 0.067038
-3.058058 0.063740
-3.048048 0.060556
-3.038038 0.057486
-3.028028 0.054528
-3.018018 0.051681
-3.008008 0.048944
-2.997998 0.046315
-2.987988 0.043793
-2.977978 0.041375
-2.967968 0.039060
-2.957958 0.036845
-2.947948 0.034728
-2.937938 0.032707
-2.927928 0.030779
-2.917918 0.028942
-2.907908 0.027193
-2.897898 0.025529
-2.887888 0.023948
-2.877878 0.022447
-2.867868 0.021024
-2.857858 0.019675
-2.847848 0.018398
-2.837838 0.017190
-2.827828 0.016049
-2.817818 0.014972
-2.807808 0.013956
-2.797798 0.012999
-2.787788 0.012098
-2.777778 0.011250
-2.767768 0.010453
-2.757758 0.009705
-2.747748 0.009004
-2.737738 0.008346
-2.727728 0.007731
-2.717718 0.007155
-2.707708 0.006617
-2.697698 0.006114
-2.687688 0.005645
-2.677678 0.005208
-2.667668 0.004801
-2.657658 0.004423
-2.647648 0.004071
-2.637638 0.003744
-2.627628 0.003440
-2.617618 0.003159
-2.607608 0.002898
-2.597598 0.002657
-2.587588 0.002434
-2.577578 0.002228
-2.567568 0.002037
-2.557558 0.001862
-2.547548 0.001700
-2.537538 0.001551
-2.527528 0.001414
-2.517518 0.001288
-2.507508 0.001173
-2.497497 0.001066
-2.487487 0.000969
-2.477477 0.000880
-2.467467 0.000799
-2.457457 0.000724
-2.447447 0.000656
-2.437437 0.000594
-2.427427 0.000537
-2.417417 0.000485
-2.407407 0.000438
-2.397397 0.000395
-2.387387 0.000357
-2.377377 0.000321
-2.367367 0.000289
-2.357357 0.000260
-2.347347 0.000234
-2.337337 0.000210
-2.327327 0.000188
-2.317317 0.000169
-2.307307 0.000151
-2.297297 0.000135
-2.287287 0.000121
-2.277277 0.000108
-2.267267 0.000097
-2.257257 0.000086
-2.247247 0.000077
-2.237237 0.000069
-2.227227 0.000061
-2.217217 0.000054
-2.207207 0.000048
-2.197197 0.000043
-2.187187 0.000038
-2.177177 0.000034
-2.167167 0.000030
-2.157157 0.000026
-2.147147 0.000023
-2.137137 0.000021
-2.127127 0.000018
-2.117117 0.000016
-2.107107 0.000014
-2.097097 0.000013
-2.087087 0.000011
-2.077077 0.000010
-2.067067 0.000009
-2.057057 0.000007
-2.047047 0.000007
-2.037037 0.000006
-2.027027 0.000005
-2.017017 0.000004
-2.007007 0.000004
-1.996997 0.000003
-1.986987 0.000003
-1.976977 0.000003
-1.966967 0.000002
-1.956957 0.000002
-1.946947 0.000002
-1.936937 0.000001
-1.926927 0.000001
-1.916917 0.000001
-1.906907 0.000001
-1.896897 0.000001
-1.886887 0.000001
-1.876877 0.000001
-1.866867 0.000001
-1.856857 0.000000
-1.846847 0.000000
-1.836837 0.000000
-1.826827 0.000000
-1.816817 0.000000
-1.806807 0.000000
-1.796797 0.000000
-1.786787 0.000000
-1.776777 0.000000
-1.766767 0.000000
-1.756757 0.000000
-1.746747 0.000000
-1.736737 0.000000
-1.726727 0.000000
-1.716717 0.000000
-1.706707 0.000000
-1.696697 0.000000
-1.686687 0.000000
-1.676677 0.000000
-1.666667 0.000000
-1.656657 0.000000
-1.646647 0.000000
-1.636637 0.000000
-1.626627 0.000000
-1.616617 0.000000
-1.606607 0.000000
-1.596597 0.000000
-1.586587 0.000000
-1.576577 0.000000
-1.566567 0.000000
-1.556557 0.000000
-1.546547 0.000001
-1.536537 0.000001
-1.526527 0.000002
-1.516517 0.000003
-1.506507 0.000005
-1.496496 0.000009
-1.486486 0.000014
-1.476476 0.000022
-1.466466 0.000035
-1.456456 0.000054
-1.446446 0.000084
-1.436436 0.000129
-1.426426 0.000197
-1.416416 0.000297
-1.406406 0.000445
-1.396396 0.000660
-1.386386 0.000970
-1.376376 0.001414
-1.366366 0.002041
-1.356356 0.002918
-1.346346 0.004133
-1.336336 0.005799
-1.326326 0.008057
-1.316316 0.011086
-1.306306 0.015107
-1.296296 0.020386
-1.286286 0.027242
-1.276276 0.036048
-1.266266 0.047232
-1.256256 0.061281
-1.246246 0.078726
-1.236236 0.100142
-1.226226 0.126128
-1.216216 0.157291
-1.206206 0.194218
-1.196196 0.237445
-1.186186 0.287423
-1.176176 0.344481
-1.166166 0.408783
-1.156156 0.480287
-1.146146 0.558715
-1.136136 0.643518
-1.126126 0.733859
-1.116116 0.828601
-1.106106 0.926321
-1.096096 1.025323
-1.086086 1.123689
-1.076076 1.219325
-1.066066 1.310038
-1.056056 1.393614
-1.046046 1.467911
-1.036036 1.530947
-1.026026 1.580993
-1.016016 1.616648
-1.006006 1.636909
-0.995996 1.641220
-0.985986 1.629493
-0.975976 1.602117
-0.965966 1.559936
-0.955956 1.504204
-0.945946 1.436529
-0.935936 1.358791
-0.925926 1.273059
-0.915916 1.181501
-0.905906 1.086290
-0.895896 0.989527
-0.885886 0.893162
-0.875876 0.798939
-0.865866 0.708348
-0.855856 0.622603
-0.845846 0.542629
-0.835836 0.469063
-0.825826 0.402277
-0.815816 0.342400
-0.805806 0.289352
-0.795796 0.242884
-0.785786 0.202614
-0.775776 0.168069
-0.765766 0.138716
-0.755756 0.113993
-0.745746 0.093339
-0.735736 0.076210
-0.725726 0.062096
-0.715716 0.050529
-0.705706 0.041091
-0.695696 0.033417
-0.685686 0.027191
-0.675676 0.022145
-0.665666 0.018056
-0.655656 0.014740
-0.645646 0.012046
-0.635636 0.009852
-0.625626 0.008062
-0.615616 0.006596
-0.605606 0.005394
-0.595596 0.004406
-0.585586 0.003592
-0.575576 0.002922
-0.565566 0.002371
-0.555556 0.001917
-0.545546 0.001544
-0.535536 0.001239
-0.525526 0.000989
-0.515516 0.000786
-0.505506 0.000622
-0.495495 0.000490
-0.485485 0.000383
-0.475475 0.000298
-0.465465 0.000231
-0.455455 0.000178
-0.445445 0.000136
-0.435435 0.000104
-0.425425 0.000078
-0.415415 0.000059
-0.405405 0.000044
-0.395395 0.000033
-0.385385 0.000024
-0.375375 0.000018
-0.365365 0.000013
-0.355355 0.000009
-0.345345 0.000007
-0.335335 0.000005
-0.325325 0.000004
-0.315315 0.000003
-0.305305 0.000002
-0.295295 0.000001
-0.285285 0.000001
-0.275275 0.000001
-0.265265 0.000000
-0.255255 0.000000
-0.245245 0.000000
-0.235235 0.000000
-0.225225 0.000000
-0.215215 0.000000
-0.205205 0.000000
-0.195195 0.000000
-0.185185 0.000000
-0.175175 0.000000
-0.165165 0.000000
-0.155155 0.000000
-0.145145 0.000000
-0.135135 0.000001
-0.125125 0.000001
-0.115115 0.000001
-0.105105 0.000001
-0.095095 0.000001
-0.085085 0.000001
-0.075075 0.000001
-0.065065 0.000001
-0.055055 0.000002
-0.045045 0.000002
-0.035035 0.000002
-0.025025 0.000003
-0.015015 0.000003
-0.005005 0.000003
0.005005 0.000004
0.015015 0.000004
0.025025 0.000005
0.035035 0.000006
0.045045 0.000006
0.055055 0.000007
0.065065 0.000008
0.075075 0.000009
0.085085 0.000011
0.095095 0.000012
0.105105 0.000014
0.115115 0.000016
0.125125 0.000018
0.135135 0.000020
0.145145 0.000023
0.155155 0.000026
0.165165 0.000029
0.175175 0.000033
0.185185 0.000037
0.195195 0.000042
0.205205 0.000047
0.215215 0.000053
0.225225 0.000060
0.235235 0.000067
0.245245 0.000075
0.255255 0.000084
0.265265 0.000095
0.275275 0.000106
0.285285 0.000118
0.295295 0.000132
0.305305 0.000148
0.315315 0.000165
0.325325 0.000184
0.335335 0.000205
0.345345 0.000229
0.355355 0.000255
0.365365 0.000283
0.375375 0.000315
0.385385 0.000349
0.395395 0.000387
0.405405 0.000429
0.415415 0.000476
0.425425 0.000526
0.435435 0.000582
0.445445 0.000643
0.455455 0.000710
0.465465 0.000783
0.475475 0.000863
0.485485 0.000951
0.495495 0.001046
0.505506 0.001151
0.515516 0.001264
0.525526 0.001388
0.535536 0.001523
0.545546 0.001669
0.555556 0.001828
0.565566 0.002001
0.575576 0.002188
0.585586 0.002391
0.595596 0.002611
0.605606 0.002848
0.615616 0.003105
0.625626 0.003382
0.635636 0.003681
0.645646 0.004003
0.655656 0.004350
0.665666 0.004723
0.675676 0.005125
0.685686 0.005555
0.695696 0.006018
0.705706 0.006513
0.715716 0.007044
0.725726 0.007613
0.735736 0.008220
0.745746 0.008869
0.755756 0.009561
0.765766 0.010300
0.775776 0.011086
0.785786 0.011924
0.795796 0.012814
0.805806 0.013760
0.815816 0.014764
0.825826 0.015829
0.835836 0.016957
0.845846 0.018151
0.855856 0.019414
0.865866 0.020748
0.875876 0.022156
0.885886 0.023641
0.895896 0.025206
0.905906 0.026853
0.915916 0.028585
0.925926 0.030404
0.935936 0.032314
0.945946 0.034316
0.955956 0.036414
0.965966 0.038609
0.975976 0.040904
0.985986 0.043301
0.995996 0.045802
1.006006 0.048410
1.016016 0.051125
1.026026 0.053950
1.036036 0.056885
1.046046 0.059933
1.056056 0.063094
1.066066 0.066370
1.076076 0.069760
1.086086 0.073264
1.096096 0.076885
1.106106 0.080620
1.116116 0.084469
1.126126 0.088432
1.136136 0.092508
1.146146 0.096695
1.156156 0.100991
1.166166 0.105394
1.176176 0.109903
1.186186 0.114513
1.196196 0.119222
1.206206 0.124026
1.216216 0.128922
1.226226 0.133905
1.236236 0.138970
1.246246 0.144113
1.256256 0.149327
1.266266 0.154608
1.276276 0.159948
1.286286 0.165342
1.296296 0.170782
1.306306 0.176261
1.316316 0.181772
1.326326 0.187306
1.336336 0.192856
1.346346 0.198413
1.356356 0.203969
1.366366 0.209514
1.376376 0.215039
1.386386 0.220535
1.396396 0.225992
1.406406 0.231400
1.416416 0.236751
1.426426 0.242032
1.436436 0.247236
1.446446 0.252352
1.456456 0.257369
1.466466 0.262278
1.476476 0.267068
1.486486 0.271731
1.496496 0.276256
1.506507 0.280633
1.516517 0.284854
1.526527 0.288910
1.536537 0.292791
1.546547 0.296489
1.556557 0.299995
1.566567 0.303303
1.576577 0.306404
1.586587 0.309291
1.596597 0.311959
1.606607 0.314399
1.616617 0.316608
1.626627 0.318580
1.636637 0.320310
1.646647 0.321794
1.656657 0.323028
1.666667 0.324011
1.676677 0.324739
1.686687 0.325210
1.696697 0.325424
1.706707 0.325380
1.716717 0.325079
1.726727 0.324520
1.736737 0.323705
1.746747 0.322637
1.756757 0.321317
1.766767 0.319749
1.776777 0.317936
1.786787 0.315884
1.796797 0.313595
1.806807 0.311077
1.816817 0.308334
1.826827 0.305373
1.836837 0.302201
1.846847 0.298825
1.856857 0.295253
1.866867 0.291491
1.876877 0.287550
1.886887 0.283437
1.896897 0.279162
1.906907 0.274733
1.916917 0.270160
1.926927 0.265453
1.936937 0.260621
1.946947 0.255675
1.956957 0.250623
1.966967 0.245476
1.976977 0.240245
1.986987 0.234939
1.996997 0.229567
2.007007 0.224141
2.017017 0.218670
2.027027 0.213163
2.037037 0.207630
2.047047 0.202081
2.057057 0.196524
2.067067 0.190968
2.077077 0.185422
2.087087 0.179895
2.097097 0.174394
2.107107 0.168927
2.117117 0.163502
2.127127 0.158126
2.137137 0.152805
2.147147 0.147547
2.157157 0.142356
2.167167 0.137239
2.177177 0.132202
2.187187 0.127248
2.197197 0.122383
2.207207 0.117610
2.217217 0.112934
2.227227 0.108358
2.237237 0.103885
2.247247 0.099518
2.257257 0.095259
2.267267 0.091109
2.277277 0.087072
2.287287 0.083147
2.297297 0.079337
2.307307 0.075641
2.317317 0.072060
2.327327 0.068594
2.337337 0.065243
2.347347 0.062007
2.357357 0.058884
2.367367 0.055875
2.377377 0.052977
2.387387 0.050190
2.397397 0.047511
2.407407 0.044940
2.417417 0.042475
2.427427 0.040112
2.437437 0.037852
2.447447 0.035690
2.457457 0.033625
2.467467 0.031654
2.477477 0.029776
2.487487 0.027986
2.497497 0.026284
2.507508 0.024665
2.517518 0.023128
2.527528 0.021669
2.537538 0.020286
2.547548 0.018977
2.557558 0.017737
2.567568 0.016566
2.577578 0.015460
2.587588 0.014416
2.597598 0.013432
2.607608 0.012505
2.617618 0.011633
2.627628 0.010813
2.637638 0.010043
2.647648 0.009321
2.657658 0.008643
2.667668 0.008009
2.677678 0.007415
2.687688 0.006860
2.697698 0.006341
2.707708 0.005857
2.717718 0.005406
2.727728 0.004985
2.737738 0.004593
2.747748 0.004229
2.757758 0.003891
2.767768 0.003577
2.777778 0.003285
2.787788 0.003015
2.797798 0.002765
2.807808 0.002534
2.817818 0.002320
2.827828 0.002123
2.837838 0.001941
2.847848 0.001773
2.857858 0.001618
2.867868 0.001476
2.877878 0.001345
2.887888 0.001224
2.897898 0.001114
2.907908 0.001013
2.917918 0.000920
2.927928 0.000835
2.937938 0.000757
2.947948 0.000686
2.957958 0.000622
2.967968 0.000562
2.977978 0.000508
2.987988 0.000459
2.997998 0.000415
3.008008 0.000374
3.018018 0.000337
3.028028 0.000303
3.038038 0.000273
3.048048 0.000246
3.058058 0.000221
3.068068 0.000198
3.078078 0.000178
3.088088 0.000159
3.098098 0.000143
3.108108 0.000128
3.118118 0.000114
3.128128 0.000102
3.138138 0.000091
3.148148 0.000081
3.158158 0.000072
3.168168 0.000064
3.178178 0.000057
3.188188 0.000051
3.198198 0.000045
3.208208 0.000040
3.218218 0.000036
3.228228 0.000032
3.238238 0.000028
3.248248 0.000025
3.258258 0.000022
3.268268 0.000019
3.278278 0.000017
3.288288 0.000015
3.298298 0.000013
3.308308 0.000012
3.318318 0.000010
3.328328 0.000009
3.338338 0.000008
3.348348 0.000007
3.358358 0.000006
3.368368 0.000005
3.378378 0.000005
3.388388 0.000004
3.398398 0.000004
3.408408 0.000003
3.418418 0.000003
3.428428 0.000002
3.438438 0.000002
3.448448 0.000002
3.458458 0.000002
3.468468 0.000001
3.478478 0.000001
3.488488 0.000001
3.498498 0.000001
3.508509 0.000001
3.518519 0.000001
3.528529 0.000001
3.538539 0.000001
3.548549 0.000000
3.558559 0.000000
3.568569 0.000000
3.578579 0.000000
3.588589 0.000000
3.598599 0.000000
3.608609 0.000000
3.618619 0.000000
3.628629 0.000000
3.638639 0.000000
3.648649 0.000000
3.658659 0.000000
3.668669 0.000000
3.678679 0.000000
3.688689 0.000000
3.698699 0.000000
3.708709 0.000000
3.718719 0.000000
3.728729 0.000000
3.738739 0.000000
3.748749 0.000000
3.758759 0.000000
3.768769 0.000000
3.778779 0.000000
3.788789 0.000000
3.798799 0.000000
3.808809 0.000000
3.818819 0.000000
3.828829 0.000000
3.838839 0.000000
3.848849 0.000000
3.858859 0.000000
3.868869 0.000000
3.878879 0.000000
3.888889 0.000000
3.898899 0.000000
3.908909 0.000000
3.918919 0.000000
3.928929 0.000000
3.938939 0.000000
3.948949 0.000000
3.958959 0.000000
3.968969 0.000000
3.978979 0.000000
3.988989 0.000000
3.998999 0.000000
4.009009 0.000000
4.019019 0.000000
4.029029 0.000000
4.039039 0.000000
4.049049 0.000000
4.059059 0.000000
4.069069 0.000000
4.079079 0.000000
4.089089 0.000000
4.099099 0.000000
4.109109 0.000000
4.119119 0.000000
4.129129 0.000000
4.139139 0.000000
4.149149 0.000000
4.159159 0.000000
4.169169 0.000000
4.179179 0.000000
4.189189 0.000000
4.199199 0.000000
4.209209 0.000000
4.219219 0.000000
4.229229 0.000000
4.239239 0.000000
4.249249 0.000000
4.259259 0.000000
4.269269 0.000000
4.279279 0.000000
4.289289 0.000000
4.299299 0.000000
4.309309 0.000000
4.319319 0.000000
4.329329 0.000000
4.339339 0.000000
4.349349 0.000000
4.359359 0.000000
4.369369 0.000000
4.379379 0.000000
4.389389 0.000000
4.399399 0.000000
4.409409 0.000000
4.419419 0.000000
4.429429 0.000000
4.439439 0.000000
4.449449 0.000000
4.459459 0.000000
4.469469 0.000000
4.479479 0.000000
4.489489 0.000000
4.499499 0.000000
4.509510 0.000000
4.519520 0.000000
4.529530 0.000000
4.539540 0.000000
4.549550 0.000000
4.559560 0.000000
4.569570 0.000000
4.579580 0.000000
4.589590 0.000000
4.599600 0.000000
4.609610 0.000000
4.619620 0.000000
4.629630 0.000000
4.639640 0.000000
4.649650 0.000000
4.659660 0.000000
4.669670 0.000000
4.679680 0.000000
4.689690 0.000000
4.699700 0.000000
4.709710 0.000000
4.719720 0.000000
4.729730 0.000000
4.739740 0.000000
4.749750 0.000000
4.759760 0.000000
4.769770 0.000000
4.779780 0.000000
4.789790 0.000000
4.799800 0.000000
4.809810 0.000000
4.819820 0.000000
4.829830 0.000000
4.839840 0.000000
4.849850 0.000000
4.859860 0.000000
4.869870 0.000000
4.879880 0.000000
4.889890 0.000000
4.899900 0.000000
4.909910 0.000000
4.919920 0.000000
4.929930 0.000000
4.939940 0.000000
4.949950 0.000000
4.959960 0.000000
4.969970 0.000000
4.979980 0.000000
4.989990 0.000000
5.000000 0.000000


==> Figures/Mixture_of_Gaussians/HOSD/pdf_hosd_p.tex <==
x pdf
-5.000000 0.000000
-4.989990 0.000000
-4.979980 0.000000
-4.969970 0.000000
-4.959960 0.000000
-4.949950 0.000000
-4.939940 0.000000
-4.929930 0.000000
-4.919920 0.000000
-4.909910 0.000000
-4.899900 0.000000
-4.889890 0.000000
-4.879880 0.000000
-4.869870 0.000000
-4.859860 0.000000
-4.849850 0.000000
-4.839840 0.000000
-4.829830 0.000000
-4.819820 0.000000
-4.809810 0.000000
-4.799800 0.000000
-4.789790 0.000000
-4.779780 0.000000
-4.769770 0.000000
-4.759760 0.000000
-4.749750 0.000000
-4.739740 0.000000
-4.729730 0.000000
-4.719720 0.000000
-4.709710 0.000000
-4.699700 0.000000
-4.689690 0.000000
-4.679680 0.000000
-4.669670 0.000000
-4.659660 0.000000
-4.649650 0.000000
-4.639640 0.000000
-4.629630 0.000000
-4.619620 0.000000
-4.609610 0.000000
-4.599600 0.000000
-4.589590 0.000000
-4.579580 0.000000
-4.569570 0.000000
-4.559560 0.000000
-4.549550 0.000000
-4.539540 0.000000
-4.529530 0.000000
-4.519520 0.000000
-4.509510 0.000000
-4.499499 0.000000
-4.489489 0.000000
-4.479479 0.000000
-4.469469 0.000000
-4.459459 0.000000
-4.449449 0.000000
-4.439439 0.000000
-4.429429 0.000000
-4.419419 0.000000
-4.409409 0.000000
-4.399399 0.000000
-4.389389 0.000000
-4.379379 0.000000
-4.369369 0.000000
-4.359359 0.000000
-4.349349 0.000000
-4.339339 0.000000
-4.329329 0.000000
-4.319319 0.000000
-4.309309 0.000000
-4.299299 0.000000
-4.289289 0.000000
-4.279279 0.000000
-4.269269 0.000000
-4.259259 0.000000
-4.249249 0.000000
-4.239239 0.000000
-4.229229 0.000000
-4.219219 0.000000
-4.209209 0.000000
-4.199199 0.000000
-4.189189 0.000000
-4.179179 0.000000
-4.169169 0.000000
-4.159159 0.000000
-4.149149 0.000000
-4.139139 0.000000
-4.129129 0.000000
-4.119119 0.000000
-4.109109 0.000000
-4.099099 0.000000
-4.089089 0.000000
-4.079079 0.000000
-4.069069 0.000000
-4.059059 0.000000
-4.049049 0.000000
-4.039039 0.000000
-4.029029 0.000000
-4.019019 0.000000
-4.009009 0.000000
-3.998999 0.000000
-3.988989 0.000000
-3.978979 0.000000
-3.968969 0.000000
-3.958959 0.000000
-3.948949 0.000000
-3.938939 0.000000
-3.928929 0.000000
-3.918919 0.000000
-3.908909 0.000000
-3.898899 0.000000
-3.888889 0.000000
-3.878879 0.000000
-3.868869 0.000000
-3.858859 0.000000
-3.848849 0.000000
-3.838839 0.000000
-3.828829 0.000000
-3.818819 0.000000
-3.808809 0.000000
-3.798799 0.000000
-3.788789 0.000000
-3.778779 0.000000
-3.768769 0.000000
-3.758759 0.000000
-3.748749 0.000000
-3.738739 0.000000
-3.728729 0.000000
-3.718719 0.000000
-3.708709 0.000000
-3.698699 0.000000
-3.688689 0.000000
-3.678679 0.000000
-3.668669 0.000000
-3.658659 0.000000
-3.648649 0.000000
-3.638639 0.000000
-3.628629 0.000000
-3.618619 0.000000
-3.608609 0.000000
-3.598599 0.000000
-3.588589 0.000000
-3.578579 0.000000
-3.568569 0.000000
-3.558559 0.000000
-3.548549 0.000000
-3.538539 0.000001
-3.528529 0.000001
-3.518519 0.000001
-3.508509 0.000001
-3.498498 0.000001
-3.488488 0.000001
-3.478478 0.000001
-3.468468 0.000001
-3.458458 0.000002
-3.448448 0.000002
-3.438438 0.000002
-3.428428 0.000002
-3.418418 0.000003
-3.408408 0.000003
-3.398398 0.000004
-3.388388 0.000004
-3.378378 0.000005
-3.368368 0.000005
-3.358358 0.000006
-3.348348 0.000007
-3.338338 0.000008
-3.328328 0.000009
-3.318318 0.000010
-3.308308 0.000012
-3.298298 0.000013
-3.288288 0.000015
-3.278278 0.000017
-3.268268 0.000019
-3.258258 0.000022
-3.248248 0.000025
-3.238238 0.000028
-3.228228 0.000032
-3.218218 0.000036
-3.208208 0.000040
-3.198198 0.000045
-3.188188 0.000051
-3.178178 0.000057
-3.168168 0.000064
-3.158158 0.000072
-3.148148 0.000081
-3.138138 0.000091
-3.128128 0.000102
-3.118118 0.000114
-3.108108 0.000128
-3.098098 0.000143
-3.088088 0.000159
-3.078078 0.000178
-3.068068 0.000198
-3.058058 0.000221
-3.048048 0.000246
-3.038038 0.000273
-3.028028 0.000303
-3.018018 0.000337
-3.008008 0.000374
-2.997998 0.000415
-2.987988 0.000459
-2.977978 0.000508
-2.967968 0.000562
-2.957958 0.000622
-2.947948 0.000686
-2.937938 0.000757
-2.927928 0.000835
-2.917918 0.000920
-2.907908 0.001013
-2.897898 0.001114
-2.887888 0.001224
-2.877878 0.001345
-2.867868 0.001476
-2.857858 0.001618
-2.847848 0.001773
-2.837838 0.001941
-2.827828 0.002123
-2.817818 0.002320
-2.807808 0.002534
-2.797798 0.002765
-2.787788 0.003015
-2.777778 0.003285
-2.767768 0.003577
-2.757758 0.003891
-2.747748 0.004229
-2.737738 0.004593
-2.727728 0.004985
-2.717718 0.005406
-2.707708 0.005857
-2.697698 0.006341
-2.687688 0.006860
-2.677678 0.007415
-2.667668 0.008009
-2.657658 0.008643
-2.647648 0.009321
-2.637638 0.010043
-2.627628 0.010813
-2.617618 0.011633
-2.607608 0.012505
-2.597598 0.013432
-2.587588 0.014416
-2.577578 0.015460
-2.567568 0.016566
-2.557558 0.017737
-2.547548 0.018977
-2.537538 0.020286
-2.527528 0.021669
-2.517518 0.023128
-2.507508 0.024665
-2.497497 0.026284
-2.487487 0.027986
-2.477477 0.029776
-2.467467 0.031654
-2.457457 0.033625
-2.447447 0.035690
-2.437437 0.037852
-2.427427 0.040112
-2.417417 0.042475
-2.407407 0.044940
-2.397397 0.047511
-2.387387 0.050190
-2.377377 0.052977
-2.367367 0.055875
-2.357357 0.058884
-2.347347 0.062007
-2.337337 0.065243
-2.327327 0.068594
-2.317317 0.072060
-2.307307 0.075641
-2.297297 0.079337
-2.287287 0.083147
-2.277277 0.087072
-2.267267 0.091109
-2.257257 0.095259
-2.247247 0.099518
-2.237237 0.103885
-2.227227 0.108358
-2.217217 0.112934
-2.207207 0.117610
-2.197197 0.122383
-2.187187 0.127248
-2.177177 0.132202
-2.167167 0.137239
-2.157157 0.142356
-2.147147 0.147547
-2.137137 0.152805
-2.127127 0.158126
-2.117117 0.163502
-2.107107 0.168927
-2.097097 0.174394
-2.087087 0.179895
-2.077077 0.185422
-2.067067 0.190968
-2.057057 0.196524
-2.047047 0.202081
-2.037037 0.207630
-2.027027 0.213163
-2.017017 0.218670
-2.007007 0.224141
-1.996997 0.229567
-1.986987 0.234939
-1.976977 0.240245
-1.966967 0.245476
-1.956957 0.250623
-1.946947 0.255675
-1.936937 0.260621
-1.926927 0.265453
-1.916917 0.270160
-1.906907 0.274733
-1.896897 0.279162
-1.886887 0.283437
-1.876877 0.287550
-1.866867 0.291491
-1.856857 0.295253
-1.846847 0.298825
-1.836837 0.302201
-1.826827 0.305373
-1.816817 0.308334
-1.806807 0.311077
-1.796797 0.313595
-1.786787 0.315884
-1.776777 0.317936
-1.766767 0.319749
-1.756757 0.321317
-1.746747 0.322637
-1.736737 0.323705
-1.726727 0.324520
-1.716717 0.325079
-1.706707 0.325380
-1.696697 0.325424
-1.686687 0.325210
-1.676677 0.324739
-1.666667 0.324011
-1.656657 0.323028
-1.646647 0.321794
-1.636637 0.320310
-1.626627 0.318580
-1.616617 0.316608
-1.606607 0.314399
-1.596597 0.311959
-1.586587 0.309291
-1.576577 0.306404
-1.566567 0.303303
-1.556557 0.299995
-1.546547 0.296489
-1.536537 0.292791
-1.526527 0.288910
-1.516517 0.284854
-1.506507 0.280633
-1.496496 0.276256
-1.486486 0.271731
-1.476476 0.267068
-1.466466 0.262278
-1.456456 0.257369
-1.446446 0.252352
-1.436436 0.247236
-1.426426 0.242032
-1.416416 0.236751
-1.406406 0.231400
-1.396396 0.225992
-1.386386 0.220535
-1.376376 0.215039
-1.366366 0.209514
-1.356356 0.203969
-1.346346 0.198413
-1.336336 0.192856
-1.326326 0.187306
-1.316316 0.181772
-1.306306 0.176261
-1.296296 0.170782
-1.286286 0.165342
-1.276276 0.159948
-1.266266 0.154608
-1.256256 0.149327
-1.246246 0.144113
-1.236236 0.138970
-1.226226 0.133905
-1.216216 0.128922
-1.206206 0.124026
-1.196196 0.119222
-1.186186 0.114513
-1.176176 0.109903
-1.166166 0.105394
-1.156156 0.100991
-1.146146 0.096695
-1.136136 0.092508
-1.126126 0.088432
-1.116116 0.084469
-1.106106 0.080620
-1.096096 0.076885
-1.086086 0.073264
-1.076076 0.069760
-1.066066 0.066370
-1.056056 0.063094
-1.046046 0.059933
-1.036036 0.056885
-1.026026 0.053950
-1.016016 0.051125
-1.006006 0.048410
-0.995996 0.045802
-0.985986 0.043301
-0.975976 0.040904
-0.965966 0.038609
-0.955956 0.036414
-0.945946 0.034316
-0.935936 0.032314
-0.925926 0.030404
-0.915916 0.028585
-0.905906 0.026853
-0.895896 0.025206
-0.885886 0.023641
-0.875876 0.022156
-0.865866 0.020748
-0.855856 0.019414
-0.845846 0.018151
-0.835836 0.016957
-0.825826 0.015829
-0.815816 0.014764
-0.805806 0.013760
-0.795796 0.012814
-0.785786 0.011924
-0.775776 0.011086
-0.765766 0.010300
-0.755756 0.009561
-0.745746 0.008869
-0.735736 0.008220
-0.725726 0.007613
-0.715716 0.007044
-0.705706 0.006513
-0.695696 0.006018
-0.685686 0.005555
-0.675676 0.005125
-0.665666 0.004723
-0.655656 0.004350
-0.645646 0.004003
-0.635636 0.003681
-0.625626 0.003382
-0.615616 0.003105
-0.605606 0.002848
-0.595596 0.002611
-0.585586 0.002391
-0.575576 0.002188
-0.565566 0.002001
-0.555556 0.001828
-0.545546 0.001669
-0.535536 0.001523
-0.525526 0.001388
-0.515516 0.001264
-0.505506 0.001151
-0.495495 0.001046
-0.485485 0.000951
-0.475475 0.000863
-0.465465 0.000783
-0.455455 0.000710
-0.445445 0.000643
-0.435435 0.000582
-0.425425 0.000526
-0.415415 0.000476
-0.405405 0.000429
-0.395395 0.000387
-0.385385 0.000349
-0.375375 0.000315
-0.365365 0.000283
-0.355355 0.000255
-0.345345 0.000229
-0.335335 0.000205
-0.325325 0.000184
-0.315315 0.000165
-0.305305 0.000148
-0.295295 0.000132
-0.285285 0.000118
-0.275275 0.000106
-0.265265 0.000095
-0.255255 0.000084
-0.245245 0.000075
-0.235235 0.000067
-0.225225 0.000060
-0.215215 0.000053
-0.205205 0.000047
-0.195195 0.000042
-0.185185 0.000037
-0.175175 0.000033
-0.165165 0.000029
-0.155155 0.000026
-0.145145 0.000023
-0.135135 0.000020
-0.125125 0.000018
-0.115115 0.000016
-0.105105 0.000014
-0.095095 0.000012
-0.085085 0.000011
-0.075075 0.000009
-0.065065 0.000008
-0.055055 0.000007
-0.045045 0.000006
-0.035035 0.000006
-0.025025 0.000005
-0.015015 0.000004
-0.005005 0.000004
0.005005 0.000003
0.015015 0.000003
0.025025 0.000003
0.035035 0.000002
0.045045 0.000002
0.055055 0.000002
0.065065 0.000001
0.075075 0.000001
0.085085 0.000001
0.095095 0.000001
0.105105 0.000001
0.115115 0.000001
0.125125 0.000001
0.135135 0.000001
0.145145 0.000000
0.155155 0.000000
0.165165 0.000000
0.175175 0.000000
0.185185 0.000000
0.195195 0.000000
0.205205 0.000000
0.215215 0.000000
0.225225 0.000000
0.235235 0.000000
0.245245 0.000000
0.255255 0.000000
0.265265 0.000000
0.275275 0.000000
0.285285 0.000000
0.295295 0.000000
0.305305 0.000000
0.315315 0.000000
0.325325 0.000000
0.335335 0.000000
0.345345 0.000000
0.355355 0.000000
0.365365 0.000000
0.375375 0.000000
0.385385 0.000000
0.395395 0.000000
0.405405 0.000000
0.415415 0.000000
0.425425 0.000000
0.435435 0.000000
0.445445 0.000001
0.455455 0.000001
0.465465 0.000001
0.475475 0.000002
0.485485 0.000004
0.495495 0.000006
0.505506 0.000010
0.515516 0.000015
0.525526 0.000024
0.535536 0.000038
0.545546 0.000059
0.555556 0.000092
0.565566 0.000140
0.575576 0.000214
0.585586 0.000322
0.595596 0.000481
0.605606 0.000713
0.615616 0.001047
0.625626 0.001523
0.635636 0.002194
0.645646 0.003131
0.655656 0.004426
0.665666 0.006198
0.675676 0.008594
0.685686 0.011803
0.695696 0.016053
0.705706 0.021620
0.715716 0.028834
0.725726 0.038079
0.735736 0.049797
0.745746 0.064480
0.755756 0.082672
0.765766 0.104954
0.775776 0.131927
0.785786 0.164197
0.795796 0.202343
0.805806 0.246888
0.815816 0.298261
0.825826 0.356760
0.835836 0.422513
0.845846 0.495432
0.855856 0.575188
0.865866 0.661176
0.875876 0.752497
0.885886 0.847958
0.895896 0.946077
0.905906 1.045112
0.915916 1.143104
0.925926 1.237933
0.935936 1.327394
0.945946 1.409282
0.955956 1.481479
0.965966 1.542046
0.975976 1.589313
0.985986 1.621956
0.995996 1.639057
1.006006 1.640152
1.016016 1.625249
1.026026 1.594831
1.036036 1.549827
1.046046 1.491568
1.056056 1.421722
1.066066 1.342215
1.076076 1.255143
1.086086 1.162682
1.096096 1.066997
1.106106 0.970163
1.116116 0.874095
1.126126 0.780487
1.136136 0.690778
1.146146 0.606122
1.156156 0.527387
1.166166 0.455156
1.176176 0.389749
1.186186 0.331250
1.196196 0.279542
1.206206 0.234348
1.216216 0.195264
1.226226 0.161801
1.236236 0.133419
1.246246 0.109555
1.256256 0.089649
1.266266 0.073162
1.276276 0.059593
1.286286 0.048483
1.296296 0.039426
1.306306 0.032065
1.316316 0.026095
1.326326 0.021257
1.336336 0.017337
1.346346 0.014156
1.356356 0.011571
1.366366 0.009465
1.376376 0.007745
1.386386 0.006336
1.396396 0.005180
1.406406 0.004230
1.416416 0.003448
1.426426 0.002803
1.436436 0.002273
1.446446 0.001836
1.456456 0.001478
1.466466 0.001185
1.476476 0.000945
1.486486 0.000751
1.496496 0.000593
1.506507 0.000466
1.516517 0.000365
1.526527 0.000284
1.536537 0.000219
1.546547 0.000169
1.556557 0.000129
1.566567 0.000098
1.576577 0.000074
1.586587 0.000056
1.596597 0.000042
1.606607 0.000031
1.616617 0.000023
1.626627 0.000017
1.636637 0.000012
1.646647 0.000009
1.656657 0.000006
1.666667 0.000005
1.676677 0.000003
1.686687 0.000002
1.696697 0.000002
1.706707 0.000001
1.716717 0.000001
1.726727 0.000001
1.736737 0.000000
1.746747 0.000000
1.756757 0.000000
1.766767 0.000000
1.776777 0.000000
1.786787 0.000000
1.796797 0.000000
1.806807 0.000000
1.816817 0.000000
1.826827 0.000000
1.836837 0.000000
1.846847 0.000000
1.856857 0.000000
1.866867 0.000001
1.876877 0.000001
1.886887 0.000001
1.896897 0.000001
1.906907 0.000001
1.916917 0.000001
1.926927 0.000001
1.936937 0.000001
1.946947 0.000002
1.956957 0.000002
1.966967 0.000002
1.976977 0.000003
1.986987 0.000003
1.996997 0.000003
2.007007 0.000004
2.017017 0.000004
2.027027 0.000005
2.037037 0.000006
2.047047 0.000007
2.057057 0.000007
2.067067 0.000009
2.077077 0.000010
2.087087 0.000011
2.097097 0.000013
2.107107 0.000014
2.117117 0.000016
2.127127 0.000018
2.137137 0.000021
2.147147 0.000023
2.157157 0.000026
2.167167 0.000030
2.177177 0.000034
2.187187 0.000038
2.197197 0.000043
2.207207 0.000048
2.217217 0.000054
2.227227 0.000061
2.237237 0.000069
2.247247 0.000077
2.257257 0.000086
2.267267 0.000097
2.277277 0.000108
2.287287 0.000121
2.297297 0.000135
2.307307 0.000151
2.317317 0.000169
2.327327 0.000188
2.337337 0.000210
2.347347 0.000234
2.357357 0.000260
2.367367 0.000289
2.377377 0.000321
2.387387 0.000357
2.397397 0.000395
2.407407 0.000438
2.417417 0.000485
2.427427 0.000537
2.437437 0.000594
2.447447 0.000656
2.457457 0.000724
2.467467 0.000799
2.477477 0.000880
2.487487 0.000969
2.497497 0.001066
2.507508 0.001173
2.517518 0.001288
2.527528 0.001414
2.537538 0.001551
2.547548 0.001700
2.557558 0.001862
2.567568 0.002037
2.577578 0.002228
2.587588 0.002434
2.597598 0.002657
2.607608 0.002898
2.617618 0.003159
2.627628 0.003440
2.637638 0.003744
2.647648 0.004071
2.657658 0.004423
2.667668 0.004801
2.677678 0.005208
2.687688 0.005645
2.697698 0.006114
2.707708 0.006617
2.717718 0.007155
2.727728 0.007731
2.737738 0.008346
2.747748 0.009004
2.757758 0.009705
2.767768 0.010453
2.777778 0.011250
2.787788 0.012098
2.797798 0.012999
2.807808 0.013956
2.817818 0.014972
2.827828 0.016049
2.837838 0.017190
2.847848 0.018398
2.857858 0.019675
2.867868 0.021024
2.877878 0.022447
2.887888 0.023948
2.897898 0.025529
2.907908 0.027193
2.917918 0.028942
2.927928 0.030779
2.937938 0.032707
2.947948 0.034728
2.957958 0.036845
2.967968 0.039060
2.977978 0.041375
2.987988 0.043793
2.997998 0.046315
3.008008 0.048944
3.018018 0.051681
3.028028 0.054528
3.038038 0.057486
3.048048 0.060556
3.058058 0.063740
3.068068 0.067038
3.078078 0.070451
3.088088 0.073979
3.098098 0.077622
3.108108 0.081380
3.118118 0.085253
3.128128 0.089238
3.138138 0.093336
3.148148 0.097545
3.158158 0.101863
3.168168 0.106288
3.178178 0.110817
3.188188 0.115447
3.198198 0.120175
3.208208 0.124998
3.218218 0.129912
3.228228 0.134912
3.238238 0.139993
3.248248 0.145150
3.258258 0.150378
3.268268 0.155671
3.278278 0.161023
3.288288 0.166426
3.298298 0.171875
3.308308 0.177361
3.318318 0.182877
3.328328 0.188415
3.338338 0.193967
3.348348 0.199525
3.358358 0.205079
3.368368 0.210621
3.378378 0.216141
3.388388 0.221630
3.398398 0.227078
3.408408 0.232475
3.418418 0.237813
3.428428 0.243080
3.438438 0.248267
3.448448 0.253363
3.458458 0.258359
3.468468 0.263245
3.478478 0.268011
3.488488 0.272647
3.498498 0.277143
3.508509 0.281490
3.518519 0.285679
3.528529 0.289700
3.538539 0.293545
3.548549 0.297206
3.558559 0.300673
3.568569 0.303940
3.578579 0.306999
3.588589 0.309843
3.598599 0.312465
3.608609 0.314860
3.618619 0.317022
3.628629 0.318945
3.638639 0.320626
3.648649 0.322061
3.658659 0.323245
3.668669 0.324177
3.678679 0.324853
3.688689 0.325273
3.698699 0.325436
3.708709 0.325341
3.718719 0.324987
3.728729 0.324377
3.738739 0.323512
3.748749 0.322393
3.758759 0.321023
3.768769 0.319406
3.778779 0.317545
3.788789 0.315445
3.798799 0.313110
3.808809 0.310546
3.818819 0.307759
3.828829 0.304756
3.838839 0.301542
3.848849 0.298126
3.858859 0.294515
3.868869 0.290717
3.878879 0.286741
3.888889 0.282595
3.898899 0.278288
3.908909 0.273830
3.918919 0.269229
3.928929 0.264497
3.938939 0.259641
3.948949 0.254672
3.958959 0.249601
3.968969 0.244437
3.978979 0.239189
3.988989 0.233869
3.998999 0.228486
4.009009 0.223050
4.019019 0.217571
4.029029 0.212058
4.039039 0.206521
4.049049 0.200970
4.059059 0.195412
4.069069 0.189858
4.079079 0.184315
4.089089 0.178792
4.099099 0.173298
4.109109 0.167839
4.119119 0.162423
4.129129 0.157057
4.139139 0.151748
4.149149 0.146503
4.159159 0.141327
4.169169 0.136225
4.179179 0.131204
4.189189 0.126267
4.199199 0.121420
4.209209 0.116667
4.219219 0.112011
4.229229 0.107455
4.239239 0.103003
4.249249 0.098657
4.259259 0.094420
4.269269 0.090293
4.279279 0.086278
4.289289 0.082376
4.299299 0.078588
4.309309 0.074915
4.319319 0.071358
4.329329 0.067915
4.339339 0.064587
4.349349 0.061373
4.359359 0.058273
4.369369 0.055286
4.379379 0.052411
4.389389 0.049645
4.399399 0.046989
4.409409 0.044439
4.419419 0.041994
4.429429 0.039652
4.439439 0.037411
4.449449 0.035269
4.459459 0.033223
4.469469 0.031271
4.479479 0.029411
4.489489 0.027639
4.499499 0.025953
4.509510 0.024351
4.519520 0.022830
4.529530 0.021386
4.539540 0.020018
4.549550 0.018723
4.559560 0.017498
4.569570 0.016340
4.579580 0.015246
4.589590 0.014215
4.599600 0.013242
4.609610 0.012327
4.619620 0.011465
4.629630 0.010656
4.639640 0.009895
4.649650 0.009182
4.659660 0.008513
4.669670 0.007887
4.679680 0.007301
4.689690 0.006753
4.699700 0.006242
4.709710 0.005764
4.719720 0.005319
4.729730 0.004904
4.739740 0.004518
4.749750 0.004160
4.759760 0.003826
4.769770 0.003517
4.779780 0.003230
4.789790 0.002964
4.799800 0.002718
4.809810 0.002490
4.819820 0.002280
4.829830 0.002085
4.839840 0.001906
4.849850 0.001741
4.859860 0.001589
4.869870 0.001449
4.879880 0.001320
4.889890 0.001202
4.899900 0.001093
4.909910 0.000994
4.919920 0.000902
4.929930 0.000819
4.939940 0.000743
4.949950 0.000673
4.959960 0.000609
4.969970 0.000551
4.979980 0.000498
4.989990 0.000450
5.000000 0.000406


==> Figures/Mixture_of_Gaussians/OSD/osd_custom_3.tex <==
% numPatterns EWvsBINARY EWvsORB EWvsHW EWvsILWO EWvsISTEP
100 28 56 49 82 58
1000 18.1 54 49.3 82.2 69.9
10000 15.22 52.77 39.6 83.67 NaN
100000 12.018 54.054 34.59 84.72 NaN
1000000 8.794 55.0058 32.4477 86.1944 NaN

